Argue with Me Tersely: Towards Sentence-Level Counter-Argument Generation

Counter-argument generation -- a captivating area in computational linguistics -- seeks to craft statements that offer opposing views. While most research has ventured into paragraph-level generation, sentence-level counter-argument generation beckons with its unique constraints and brevity-focused challenges. Furthermore, the diverse nature of counter-arguments poses challenges for evaluating model performance solely based on n-gram-based metrics. In this paper, we present the ArgTersely benchmark for sentence-level counter-argument generation, drawing from a manually annotated dataset from the ChangeMyView debate forum. We also propose Arg-LlaMA for generating high-quality counter-argument. For better evaluation, we trained a BERT-based evaluator Arg-Judge with human preference data. We conducted comparative experiments involving various baselines such as LlaMA, Alpaca, GPT-3, and others. The results show the competitiveness of our proposed framework and evaluator in counter-argument generation tasks. Code and data are available at https://github.com/amazingljy1206/ArgTersely.

==> Appendices/temp6.tex <==
\section{More Information about the Annotation Process}
\label{annotation process}

The dataset was enhanced through thorough annotation of the CMV dataset. Within CMV, a quoting dynamic exists: user B selects a part of user A's statement (usually a sentence) and responds to it (often multiple sentences). These sentence pairs with quoting relations were defined as "conversations," serving as annotation source data. User A's statement is the original argument, and annotators extract concise expressions (single sentence) from user B's replies as sentence-level counter-argument.

Before presenting conversations and topics to annotators, we preprocessed the source data. User B's replies were segmented into candidate sentences using punctuation marks, and sentences containing hyperlinks, emails, phone numbers, emojis, etc., were removed (which protects the privacy of users). After that, grammar errors (capitalization, spacing) were corrected.

Annotators selected sentences from the candidate set that convincingly refuted the original argument. An option to invalidate conversations was provided, applicable if the original argument was syntactically incomplete, lacked a specific viewpoint, or contained harmful content.

Prior to formal annotation, annotators underwent training which included understanding annotation rules and the system, as well as sensitivity towards invalidating conversations. After training, annotators conducted trial annotations. Consistency between our self-annotations and each annotator's results was assessed, retaining those with good consistency for formal annotation (24 annotators at last). During formal annotation, two annotators cross-evaluated each content piece. If a candidate sentence was unanimously selected or not by both annotators, it became a sentence-level counter-argument. Otherwise, a third annotator arbitrated and determined the final result. About 30\% of the corpus is generated by arbitration. Invalid conversations were promptly removed during the annotation process if an annotator deemed them unfit. The annotation process lasted 42 days.

==> Figures/04case_study.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.5\textwidth]{Figures/case_study.pdf}
    \caption{Case study of an instance in the test set. Our model produces more appropriate counter-arguments.}
    \label{case_study}
\end{figure}

==> Sections/22arg_tersely_old.tex <==
\subsection{Dataset Creation}

Our dataset is sourced from Change- MyView (CMV), a subcommunity on Reddit where users submit posts expressing their perspectives on various topics. In CMV, users engage in debates to challenge and potentially change the original posters’ views. The annotation work for our dataset is based on the CMV dataset~\cite{cmv_base}, which includes the citation relationship between original posts and their corresponding replies. We initially extracted 20,626 conversations from the dataset focusing on the reply relationship. Each conversation comprises a topic, an original argument, and its corresponding reply. Notably, the original argument is a sentence, while the reply may be a paragraph. The main steps we took to obtain the dataset are as follows:
\begin{enumerate}
    \item We divided the replies into multiple candidate sentences using ending symbols like periods and question marks.
    \item The candidate sentences underwent a cleaning process where we removed hyperlinks, non-English characters, and unwanted elements. We also applied spelling standardization, including capitalizing the first letter.
    \item We asked annotators to identify sentences from the split candidates that formed a rebuttal relationship with the original argument, considering the topic. Each identified sentence was considered a counter-argument.
\end{enumerate}

We enlisted a group of $24$ annotators, all with extensive experience in debate competitions and holding a minimum of a bachelor’s degree. We finally obtained $31,197$ pairs of arguments and their corresponding counter-arguments, each associated with the relevant topic. Detailed introductions to the annotation process are in Appendix. The statistics of ArgTersely are shown in Table~\ref{argtersely_desc}.


